Few-Shot Text Ranking with Meta Adapted Synthetic Weak Supervision

The effectiveness of Neural Information Retrieval (Neu-IR) often depends on a large scale of in-domain relevance training signals, which are not always available in real-world ranking scenarios. To democratize the benefits of Neu-IR, this paper presents MetaAdaptRank, a domain adaptive learning method that generalizes Neu-IR models from label-rich source domains to few-shot target domains. Drawing on source-domain massive relevance supervision, MetaAdaptRank contrastively synthesizes a large number of weak supervision signals for target domains and meta-learns to reweight these synthetic "weak" data based on their benefits to the target-domain ranking accuracy of Neu-IR models. Experiments on three TREC benchmarks in the web, news, and biomedical domains show that MetaAdaptRank significantly improves the few-shot ranking accuracy of Neu-IR models. Further analyses indicate that MetaAdaptRank thrives from both its contrastive weak data synthesis and meta-reweighted data selection. The code and data of this paper can be obtained from https://github.com/thunlp/MetaAdaptRank.

==> Archive/4_Experiment_Settings_old.tex <==
\section{Experiment Settings}

This section describes our experimental settings and implementation details.

% ******************************************
% ******************************************

\textbf{Evaluation Benchmarks.} Three few-shot TREC benchmarks of different domains are used in our experiments, and the details are listed in Table~\ref{tab:dataset}. ClueWeb09-B is a web domain dataset, which contains 200 labeled queries and over 50 million documents. Robust04 consists of 249 labeled queries and over 500k news articles. TREC-COVID is a recently published dataset, targeting literature search with COVID-related biomedical papers. The ``Complete'' version of TREC-COVID is used, which consists of 50 annotated queries. 

% The ``Complete'' version of TREC-COVID consists of 50 annotated queries and is used. 

We inherited the same reranking settings on ClueWeb09 and Robust04 from the previous related works~\cite{dai2019deeper, zhang2020selective} for fair comparisons, which rerank the top 100 documents from SDM and five-fold cross-validation with the exactly same fold splits.  With consistent benchmarking, all our results on ClueWeb09 and Robust04 are directly comparable with those reported in previous research~\cite{zhang2020selective, dai2019deeper, xiong2017duet}. In TREC-COVID, we rerank the top 100 with five-fold cross-validation, but from Anserini BM25\footnote{https://github.com/castorini/anserini}, which is extensively adopted as the first-stage retrieval in TREC-COVID task~\cite{macavaney2020sledge, almeida2020frugal, xiong2020cmt, mass2020ad}. 
%Our results on ClueWeb09 and Robust04 are thus directly comparable with all reported in Dai et al.~\cite{dai2019deeper} and Zhang et al.~\cite{zhang2020selective}. This consistent benchmarking is crucial for reproducibility and avoids comparing with weaker baselines, as pointed out by Yang et al.~\cite{yang2019critically}. We will include these data resources, pre-processing scripts, intermediate data, and benchmarking numbers in our open source repository.


% ******************************************
% ******************************************

\textbf{Evaluation Metrics.} NDCG@20~\cite{jarvelin2002cumulated} is used on all datasets and regarded as our main evaluation metric. In addition, following previous work~\cite{dai2019deeper, zhang2020selective}, ERR@20~\cite{chapelle2009expected} is used on ClueWeb09-B and Robust04. P@20 is used on TREC-COVID, which is provided by the official evaluation. Statistic significance is tested by permutation test with $p<0.05$.


% There are two selection criteria for the evaluation indicators on the above three data sets. One is the official evaluation metrics. The other is consistent with the previous related work settings for a fair comparison. On all benchmarks, We inherit the exact same fold splits and the same evaluation metrics:  NDCG@20, ERR@20, and permutation test with $p<0.05$ for statistical significance test. 

% ******************************************
% ******************************************


%% ********************************
\input{Diagrams/datasets}
%% ********************************


\textbf{Baselines.} Two groups of baselines are compared to verify our weak supervised learning framework's effectiveness, including \textit{Traditional IR models} and \textit{Neu-IR models}.

\textit{Traditional IR.} Following previous work~\cite{dai2019deeper, zhang2019generic}, two unsupervised IR methods, BM25~\cite{robertson2009probabilistic} and Sequential Dependency Model (SDM)~\cite{metzler2005markov}, are compared in our experiments. In addition, RankSVM~\cite{joachims2002optimizing} and Coordinate Ascent (Coor-Ascent)~\cite{metzler2007linear}, are also compared, which are the best feature-based learning to rank results reported on this benchmark setting~\cite{dai2019deeper, zhang2019generic}.

\textit{Neu-IR models}. 
In our experiments, we mainly conduct experiments with BERT~\cite{devlin2019bert}, which has shown robust performance on the above three ranking benchmarks~\cite{dai2019deeper, zhang2020selective, mass2020ad}. For TREC-COVID, we use PubMedBERT~\cite{pubmedbert}, a biomedical-domain language model trained with PubMed articles. 

To further evaluate the effectiveness of our models, several weak supervision methods are employed as our baselines. For two ad-hoc retrieval datasets, ClueWeb09-B and Robust04, we borrow results from two baselines, Bing User Click~\cite{dai2019deeper} and Title-Doc Filter~\cite{macavaney2019content}, which train Neu-IR models with Bing user clicks and filtered title-document pairs, respectively. For all datasets, we train Neu-IR models with anchor-document relations~\cite{zhang2020selective} and MS MARCO Human Label~\cite{msmarco}, a large-scale ad-hoc ranking dataset that includes one million human-labeled queries from Bing. QG~\cite{ma2020zero} is also compared in our experiments. QG generates queries with in-domain documents and regards the synthetic query-document pairs as weak supervision data. The recent weak supervision selection method, ReInfoSelect~\cite{zhang2020selective}, is also regarded as our baseline. It uses reinforcement learning to better select weak supervisions for training and achieves promising results on all benchmarks~\cite{zhang2020selective,xiong2020cmt}.

%% ********************************
\input{Diagrams/overall}
%% ********************************

%% *****************************
\input{Diagrams/bleu_score}
\input{Diagrams/weak_data}
%% *****************************



% ******************************************
% ******************************************

\textbf{Implementation Details.}
The rest of this section describes our implementation details. All our models are implemented with PyTorch. T5, BERT, and PubMedBERT inherit huggingface's implementation\footnote{https://github.com/huggingface/pytorch-transformers}. Adam optimizer is used to optimize all parameters with a learning rate of 2e-5. 

\textit{ContrastQG.} We employ T5~\cite{raffel2020exploring} as our query generator, which is same as~\citet{lu2020neural}. We use the small version of T5 and set the maximum input length and batch size to 512 and 4, respectively. ContrastQG uses BM25 to retrieve negative documents ($d^-$). During training, we use MS MARCO~\cite{msmarco} to train the query generator. And the greedy search is used during inference to generate pseudo queries.



\textit{Neu-IR Models.} In our experiments, we use the base version of BERT and PubMedBERT and keep all hyperparameters the same as prior work~\cite{zhang2020selective} and use their open-source implementations from OpenMatch\footnote{https://github.com/thunlp/OpenMatch}. We set the max input length to 512 and batch size to 8. In ClueWeb09-B and Robust04, we use Coor-Ascent to aggregate the ranking features from Neu-IR models with the first-stage retrieval score, following previous research~\cite{convknrm, dai2019deeper, zhang2020selective}.
The same neural ranker is trained with only a few-shot label data from benchmarks without extra weak supervision training data. This is our vanilla baseline. We respectively report our implementation results and scores from the previous work~\cite{zhang2020selective}.



We keep consistent with the prior work~\cite{dai2019deeper, zhang2020selective, lu2020neural} to train our models with weak supervision data. The neural ranker is first trained with weak supervision signals and is continuously fine-tuned on few-shot target benchmarks. For \meta{}, We set the batch size of weak supervision data ($n$) and few-shot target data ($m$) to 8.



 





==> Archive/bleu.tex <==
\begin{table}[]
\resizebox{80mm}{16mm}{
\begin{tabular}{llllll}
\hline
Setting          & BLEU@1          & BLEU@2          & NIST@1          & NIST@2          & METEOR          \\ \hline
\multicolumn{6}{l}{\textbf{MSMarco}}                                                                                \\ \hline
QG               & 0.5672          & 0.4527          & 5.8070          & 7.3315          & 0.3089          \\
Contrast         & \textbf{0.5909} & \textbf{0.4627} & \textbf{6.1282} & \textbf{7.6314} & \textbf{0.3191} \\
reverse Contrast & 0.3185          & 0.1807          & 3.0076          & 3.3665          & 0.1610          \\ \hline
\multicolumn{6}{l}{\textbf{MedMarco}}                                                                               \\ \hline
QG               & 0.6407          & 0.5544          & 6.2276          & 8.2823          & 0.3674          \\
Contrast         & \textbf{0.6523} & \textbf{0.5610} & \textbf{6.3977} & \textbf{8.4582} & \textbf{0.3729} \\
reverse Contrast & 0.2699          & 0.1479          & 2.3929          & 2.6468          & 0.1355          \\ \hline
\end{tabular}
}
\caption{The score of automatic evaluation metric on a held-out set of 10K MSMarco triples. In \textbf{reverse Contrast}, we swap the document pair, using the previous negative document as positive document}
\end{table}

==> Archive/contrast_vs_qg.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.88}{
  \begin{tabular}{l c c c}
  \toprule
  \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{NDCG@20}} \\
  & \textbf{ClueWeb09-B} & \textbf{Robust04} & \textbf{TREC-COVID} \\
  \hline
  Anhcor & 0.3072 & 0.4446 & n.a. \\
  QG & 0.3036 & 0.4685 & 0.7866 \\
  \textbf{ContrastQG} & \textbf{0.3124} & \textbf{0.4769} & \textbf{0.7908} \\
  \bottomrule
  \end{tabular}
  }
  \caption{\label{tab:qg_ndcg}}
\end{table}

==> Archive/name.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.93}{
\begin{tabular}{l l|l|l}
% \begin{tabularx}{\textwidth}{lXXX}
  \toprule
  \multicolumn{2}{l|}{\textbf{Synthetic Query}} & \textbf{Positive Document} & \textbf{Negative Document} \\ 
    \hline
    % \multirow{2}{*}{(+)} & what is \textbf{\textcolor{red}{microsoft}} malicious removal tool (ContrastQG) \\
    % \hline
    
    \multirow{2}{*}{(+)} & 
    \tabincell{l}{what is \redbf{microsoft} malicious removal tool (\textit{ContrastQG}) \\
    what is the malicious \bluebf{software} removal tool (\textit{QG})} & 
    
    \tabincell{l}{
    … microsoft malicious software removal tool microsoft \\ 
    windows malicious software removal tool checks computers \\
    running windows xp, windows 2000, and windows server 2003 \\
    for infections by specific, prevalent malicious software including blaster, sasser, and mydoom … malicious software was detected and removed. download : microsoft malicious software removal tool ...} & 
    \tabincell{l}{… microsoft malicious software removal tool microsoft windows malicious software removal tool checks computers running windows xp, windows 2000, and windows server 2003 for infections by specific, prevalent malicious software including blaster, sasser, and mydoom … malicious software was detected and removed. download : microsoft malicious software removal tool ...}
    \\
    
    
    % \hline
    % what is the malicious \textcolor{blue}{software} removal tool (QG)
    
    % & \textcolor{red}{microsoft} malicious \textcolor{blue}{software} removal tool \textcolor{red}{microsoft} windows malicious \textcolor{blue}{soft-}
    % & … all tips buying guide forum downloads news reviews home forum wind-  \\
    
    % what is \textcolor{red}{microsoft} malicious removal tool (\textbf{ContrastQG}) 
    % & \textcolor{blue}{ware} removal tool checks computers running windows xp, windows 2000, and windows server 2003 for infections by specific, prevalent malicious \textcolor{blue}{software} including … malicious \textcolor{blue}{software} was detected and removed. download : \textcolor{red}{microsoft} malicious \textcolor{blue}{software} removal tool…
    % & ows forum linux forum macos forum hardware forum \textcolor{blue}{software} forum videogames forum office \textcolor{blue}{software} forum programing forum webmastering… \\
    
    
    % when did the usc \textcolor{blue}{trojans} start (QG) 
    % & 2004 \textcolor{red}{usc} \textcolor{blue}{trojans} \textcolor{red}{football team}, the free 
    % & … about how the \textcolor{blue}{trojan} war began the  \\
    % what is the \textcolor{red}{usc football team} (\textbf{ContrastQG}) 
    % & encyclopedia the 2004 \textcolor{red}{usc} \textcolor{blue}{trojans} \textcolor{red}{football team} represented the university of southern california in the 2004-2005 ncaa division i-a college \textcolor{red}{football} season …
    % & aftermath of the \textcolor{blue}{trojan} war. comment how the \textcolor{blue}{trojan} war began like the \textcolor{blue}{trojan} war, the persian wars were a defining moment in greek history for all their importance, though…\\
    
    % \hline
    % what is \textcolor{blue}{green energy} ecosystem (QG)
    % & \textcolor{blue}{green} at \textcolor{red}{msn} shopping \textcolor{red}{shopping with}  
    % & …  what you can do \textcolor{blue}{energy} star pledge  \\
    
    % how does \textcolor{red}{shopping with the planet make} \textcolor{red}{a big difference in msn} eco (\textbf{ContrastQG}) 
    % & \textcolor{red}{the planet} in mind can \textcolor{red}{make a big difference} by \textcolor{red}{msn} shopping msn \textcolor{blue}{green} am \textcolor{red}{shopping with the planet} in mind can \textcolor{red}{make a big difference} in myriad ways. … reduce the amount of toxic materials entering our ecosystems. \textcolor{blue}{energy} saving solutions conserving \textcolor{blue}{energy} reduces co2 emissions…
    % & donate resources boater guide marinas harbormasters pump outs public beaches fishing hot spots boating practices boater safety conservation news and events practical conservation overview \textcolor{blue}{green} thumb ride share candle light dinner bright idea … \\

    \bottomrule
\end{tabular}
% \end{tabularx}
}
\caption{Case Studies of synthetic queries. The \textcolor{blue}{blue} texts are shared by the two documents, and the \textcolor{red}{red} texts are the specific content of the positive document.
}
\end{table*}


==> Archive/old_case_examples.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.93}{
% \begin{tabularx}{\textwidth}{XXX}
\begin{tabular}{l l|l|l}
  \toprule
  \textbf{Synthetic Queries} & \textbf{Positive Document} & \textbf{Negative Document} \\ 
    \hline
    when did the usc \textcolor{blue}{trojans} start (QG) 
    & 2004 \textcolor{red}{usc} \textcolor{blue}{trojans} \textcolor{red}{football team}, the free 
    & … about how the \textcolor{blue}{trojan} war began the  \\
    what is the \textcolor{red}{usc football team} (\textbf{ContrastQG}) 
    & encyclopedia the 2004 \textcolor{red}{usc} \textcolor{blue}{trojans} \textcolor{red}{football team} represented the university of southern california in the 2004-2005 ncaa division i-a college \textcolor{red}{football} season …
    & aftermath of the \textcolor{blue}{trojan} war. comment how the \textcolor{blue}{trojan} war began like the \textcolor{blue}{trojan} war, the persian wars were a defining moment in greek history for all their importance, though…\\
    
    \hline
    what is \textcolor{blue}{green energy} ecosystem (QG)
    & \textcolor{blue}{green} at \textcolor{red}{msn} shopping \textcolor{red}{shopping with}  
    & …  what you can do \textcolor{blue}{energy} star pledge  \\
    
    how does \textcolor{red}{shopping with the planet make} \textcolor{red}{a big difference in msn} eco (\textbf{ContrastQG}) 
    & \textcolor{red}{the planet} in mind can \textcolor{red}{make a big difference} by \textcolor{red}{msn} shopping msn \textcolor{blue}{green} am \textcolor{red}{shopping with the planet} in mind can \textcolor{red}{make a big difference} in myriad ways. … reduce the amount of toxic materials entering our ecosystems. \textcolor{blue}{energy} saving solutions conserving \textcolor{blue}{energy} reduces co2 emissions…
    & donate resources boater guide marinas harbormasters pump outs public beaches fishing hot spots boating practices boater safety conservation news and events practical conservation overview \textcolor{blue}{green} thumb ride share candle light dinner bright idea … \\
    
    \hline
    what is the malicious \textcolor{blue}{software} removal tool (QG)
    & \textcolor{red}{microsoft} malicious \textcolor{blue}{software} removal tool \textcolor{red}{microsoft} windows malicious \textcolor{blue}{soft-}
    & … all tips buying guide forum downloads news reviews home forum wind-  \\
    
    what is \textcolor{red}{microsoft} malicious removal tool (\textbf{ContrastQG}) 
    & \textcolor{blue}{ware} removal tool checks computers running windows xp, windows 2000, and windows server 2003 for infections by specific, prevalent malicious \textcolor{blue}{software} including … malicious \textcolor{blue}{software} was detected and removed. download : \textcolor{red}{microsoft} malicious \textcolor{blue}{software} removal tool…
    & ows forum linux forum macos forum hardware forum \textcolor{blue}{software} forum videogames forum office \textcolor{blue}{software} forum programing forum webmastering… \\
    
    \bottomrule
\end{tabular}
% \end{tabularx}
}
\caption{Case Studies of synthetic queries. The \textcolor{blue}{blue} texts are shared by the two documents, and the \textcolor{red}{red} texts are the specific content of the positive document.
}
\end{table*}


==> Archive/overall-2.tex <==
\begin{table*}[t]
\centering
\small
  \caption{\label{tab:overall}Overall Ranking Accuracy.}
  \begin{tabular}{l|l l|l l|l l}
  \toprule
  \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{ClueWeb09-B}} & \multicolumn{2}{c|}{\textbf{Robust04}} & \multicolumn{2}{c}{\textbf{TREC-COVID R5}} \\
   & \textbf{NDCG@20} & \textbf{ERR@20} & \textbf{NDCG@20} & \textbf{ERR@20} & \textbf{NDCG@20} & \textbf{P@20} \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{No Weak Supervision}}} \\
   \midrule
   Base Retrieval & 0.2774 & 0.1380 & 0.4272 & 0.1172 & 0.5941 & 0.6410 \\
   No Weak Supervision \cite{zhang2020selective} & 0.2999 & 0.1631 & 0.4258 & 0.1163 & n.a. & n.a. \\
   No Weak Supervision (Ours) & Q & Q & Q & Q & \textbf{0.7294} & \textbf{0.7720} \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{Full Weak Supervision}}} \\
   \midrule
   Bing User Click~\cite{dai2019deeper} & 0.333 & n.a. & n.a. & n.a. & n.a. & n.a. \\
   Anchor~\cite{zhang2020selective} & 0.3072 & 0.1609 & 0.4446 & 0.1206 & Q & Q \\
%   Ms Marco Human Label \cite{zhang2020selective} & 0.3085 & 0.1652 & 0.4415 & 0.1213 & n.a. & n.a. \\
   Ms Marco Human Label (Ours) & Q & Q & Q & Q & Q & Q \\
   \hline
   QG~\cite{ma2020zero} & Q & Q & Q & Q & Q & Q \\
   ContrastQG & Q & Q & Q & Q & Q & Q \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{Selective Weak Supervision}}} \\
   \midrule
   ReInfoSelect (Anchor)\cite{zhang2020selective} & 0.3261 & 0.1669 & 0.4500 & 0.1220 & Z & Z \\
   MetaLeToR (Anchor) & \textbf{0.3374} & \textbf{0.1730} & \textbf{0.4797} & \textbf{0.1314} & S & S\\
   \hline
   ReInfoSelect (Marco) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (Marco) & S & S & S & S & S & S \\
   \hline
   ReInfoSelect (QG) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (QG) & S & S & S & S & S & S \\
   \hline
   ReInfoSelect (ContrastQG) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (ContrastQG) & S & S & S & S & S & S \\
    \bottomrule
  \end{tabular}
\end{table*}


==> Archive/overall-old.tex <==
\begin{table*}[t]
\centering
\small
  \caption{\label{tab:overall}Overall Ranking Accuracy.}
  \begin{tabular}{l|l l|l l|l l}
  \toprule
  \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{ClueWeb09-B}} & \multicolumn{2}{c|}{\textbf{Robust04}} & \multicolumn{2}{c}{\textbf{TREC-COVID R5}} \\
   & \textbf{NDCG@20} & \textbf{ERR@20} & \textbf{NDCG@20} & \textbf{ERR@20} & \textbf{NDCG@20} & \textbf{P@20} \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{No Weak Supervision}}} \\
   \midrule
   Base Retrieval & 0.2774 & 0.1380 & 0.4272 & 0.1172 & 0.5941 & 0.6410 \\
   No Weak Supervision \cite{zhang2020selective} & 0.2999 & 0.1631 & 0.4258 & 0.1163 & n.a. & n.a. \\
   No Weak Supervision (Ours) & Q & Q & Q & Q & \textbf{0.7294} & \textbf{0.7720} \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{Full Weak Supervision}}} \\
   \midrule
   Bing User Click~\cite{dai2019deeper} & 0.333 & n.a. & n.a. & n.a. & n.a. & n.a. \\
   Anchor~\cite{zhang2020selective} & 0.3072 & 0.1609 & 0.4446 & 0.1206 & Q & Q \\
   Ms Marco Human Label \cite{zhang2020selective} & 0.3085 & 0.1652 & 0.4415 & 0.1213 & n.a. & n.a. \\
   Ms Marco Human Label (Ours) & Q & Q & Q & Q & Q & Q \\
   \hline
   QG~\cite{ma2020zero} & 0.3306 & 0.1748 & 0.4735 & 0.1301 & Q & Q \\
   ContrastQG & 0.3333 & 0.1864 & 0.4829 & 0.1304 & 0.7445 & 0.7760 \\
   \midrule
   \multicolumn{7}{l}{\textbf{\textsc{Selective Weak Supervision}}} \\
   \midrule
   ReInfoSelect (Anchor)\cite{zhang2020selective} & 0.3261 & 0.1669 & 0.4500 & 0.1220 & Z & Z \\
   MetaLeToR (Anchor) & \textbf{0.3374} & \textbf{0.1730} & \textbf{0.4797} & \textbf{0.1314} & S & S\\
   \hline
   ReInfoSelect (Marco) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (Marco) & S & S & S & S & 0.7814 & 0.8210 \\
   \hline
   ReInfoSelect (QG) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (QG) & S & S & S & S & S & S \\
   \hline
   ReInfoSelect (ContrastQG) & Z & Z & Z & Z & Z & Z \\
   MetaLeToR (ContrastQG) & 0.3435 & 0.1824 & 0.4916 & 0.1362 & S & S \\
    \bottomrule
  \end{tabular}
\end{table*}


==> Diagrams/contrastqg_vs_marco.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.92}{
  \begin{tabular}{l|c}
  \toprule
  \textbf{Methods} & \textbf{NDCG@20} \\
  \hline
  \meta{} (All Marco) & \textbf{0.8354} \\
  \meta{} (ContrastQG $\Leftarrow$ All Marco) & 0.8341 \\
  \hline
  \meta{} (1\% Marco) & run \\
  \meta{} (ContrastQG $\Leftarrow$ 1\% Marco) & run \\
  \bottomrule
  \end{tabular}
  }
  \caption{\label{tab:adaptive_ndcg}The NDCG@20 results on TREC-COVID with different proportions of weakly supervised data. 1\% Marco denotes that we takes 1\% MS MARCO human labels for model training. ContrastQG $\Leftarrow$ 1\% Marco denotes that we first uses 1\% MS MARCO data to train ContrastQG, and then train the ranker on the COVID-domain weak labels generated by ContrastQG.}
\end{table}

% \begin{table}[t]
% \centering
% \small
% \scalebox{0.92}{
%   \begin{tabular}{l c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{TREC-COVID}} \\
%   & \textbf{NDCG@20} & \textbf{P@20} \\
%   \hline
%   \textbf{100\%} MARCO Human Labels & 0.8057 & 0.8570 \\
%   ContrastQG & 0.7908 & 0.8580 \\
%   \textbf{\meta{} (ContrastQG)} & \textbf{0.8341} & \textbf{0.8780} \\
%   \hline
%   \textbf{1\%} MARCO Human Labels & 0.7915 & 0.8430 \\
%   ContrastQG & \textbf{0.7941} & \textbf{0.8500} \\
%   \textbf{\meta{} (ContrastQG)} & run & run \\
%   \bottomrule
%   \end{tabular}
%   }
%   \caption{\label{tab:adaptive_ndcg}The adaptive performance of \meta{} and ReInfoSelect for different weakly supervised data (anchor and synthetic data from ContrastQG).}
% \end{table}


% \begin{table}[t]
% \centering
% \small
% \scalebox{0.7}{
%   \begin{tabular}{l|c c|c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{100\% MARCO}} & \multicolumn{2}{c}{\textbf{1\% MARCO}} \\
%   & NDCG@20 & P@20 & NDCG@20 & P@20\\
%   \hline
%   MS MARCO & 0.8057 & 0.8570 & - & - \\
%   ContrastQG & 0.7908 & 0.8580 & - & - \\
%   MetaLTR (ContrastQG) & 0.8341 & 0.8780 & - & - \\
%   \bottomrule
%   \end{tabular}
%   }
%   \caption{\label{tab:adaptive_ndcg}The adaptive performance of \meta{} and ReInfoSelect for different weakly supervised data (anchor and synthetic data from ContrastQG).}
% \end{table}



% \begin{table*}[t]
% \centering
% \small
% \scalebox{0.92}{
%   \begin{tabular}{l|c c|c c|c c|c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{100\% Marco}} & \multicolumn{2}{c|}{\textbf{5k Marco}} & \multicolumn{2}{c|}{\textbf{3k Marco}} & \multicolumn{2}{c}{\textbf{1k Marco}} \\
%   & NDCG@20 & P@20 & NDCG@20 & P@20 & NDCG@20 & P@20 & NDCG@20 & P@20 \\
%   \hline
%   \meta{} (MARCO) & - & - & - & - & - & - & - & - \\
%   \meta{} (ContrastQG) & - & - & - & - & - & - & - & - \\
%   \bottomrule
%   \end{tabular}
%   }
%   \caption{\label{tab:adaptive_ndcg}The adaptive performance of \meta{} and ReInfoSelect for different weakly supervised data (anchor and synthetic data from ContrastQG).}
% \end{table*}


==> Diagrams/contrastqg_vs_qg.tex <==
\begin{table}[h]
\centering
\small
\scalebox{0.85}{
  \begin{tabular}{l|c c c}
  \toprule
  \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{NDCG@20}} \\
  & \textbf{ClueWeb09-B} & \textbf{Robust04} & \textbf{TREC-COVID} \\
  \hline
  \multicolumn{4}{l}{\textbf{Human-access}} \\
  \hline
  Bing User Click & \textbf{0.333} & n.a & n.a. \\
  Anchor & 0.3072 & 0.4446 & n.a. \\
  MS MARCO & 0.3205 & \textbf{0.4674} & \textbf{0.8057} \\
  \hline
  \multicolumn{8}{l}{\textbf{Auto-synthesis}} \\
  \hline
  QG & 0.3036 & 0.4685 & 0.7866  \\
  \textbf{ContrastQG} & \textbf{0.3123} & \textbf{0.4769} & \textbf{0.7908} \\
  \bottomrule
  \end{tabular}
  }
  \caption{\label{tab:contrastqg}The ranking performance with different weakly supervised sources and the quality of queries generated from synthetic methods. We only report NDCG@20 due to the space limit.}
\end{table}


% \begin{table*}[t]
% \centering
% \small
% \scalebox{0.92}{
%   \begin{tabular}{l|c c c|c c c c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{NDCG@20}} & \multicolumn{5}{c}{\textbf{Generation Quality}} \\
%   & \textbf{ClueWeb09-B} & \textbf{Robust04} & \textbf{TREC-COVID} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{NIST-1} & \textbf{NIST-2} & \textbf{METEOR} \\
%   \hline
%   \multicolumn{8}{l}{\textbf{Human-access}} \\
%   \hline
%   Bing User Click & 0.333 & n.a & n.a. & n.a. & n.a. & n.a. & n.a. & n.a. \\
%   Anchor & 0.3072 & 0.4446 & n.a. & n.a. & n.a. & n.a. & n.a. & n.a.  \\
%   MS MARCO & 0.3205 & 0.4674 & 0.8057 & n.a. & n.a. & n.a. & n.a. & n.a. \\
%   \hline
%   \multicolumn{8}{l}{\textbf{Automatic-synthesis}} \\
%   \hline
%   QG & 0.3036 & 0.4685 & 0.7866 & 0.5672 & 0.4527 & 5.8070 & 7.3315 & 0.3089 \\
%   \textbf{ContrastQG} & \textbf{0.3123} & \textbf{0.4769} & \textbf{0.7908} & \textbf{0.5909} & \textbf{0.4627} & \textbf{6.1282} & \textbf{7.6314} & \textbf{0.3191} \\
%   \textbf{reverse} ContrastQG & n.a. & n.a. & n.a. & 0.3185 & 0.1807 & 3.0076 & 3.3665 & 0.1610 \\
%   \bottomrule
%   \end{tabular}
%   }
%   \caption{\label{tab:contrastqg}The ranking performance with different weakly supervised sources and the quality of queries generated from synthetic methods. In \textbf{reverse} ContrastQG, we swap the encoding position of contrast document pair, using the previous negative document as positive document. We only report NDCG@20 due to the space limit.}
% \end{table*}


% \begin{table*}[t]
% \centering
% \small
% \scalebox{0.92}{
%   \begin{tabular}{l|c c c c c|c c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c|}{\textbf{Generation Quality}} & \multicolumn{3}{c}{\textbf{Ranking NDCG@20}} \\
%   & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{NIST-1} & \textbf{NIST-2} & \textbf{METEOR} &  \textbf{ClueWeb09-B} & \textbf{Robust04} & \textbf{TREC-COVID} \\
%   \hline
%   Anchor & n.a. & n.a. & n.a. & n.a. & n.a. & 0.3072 & 0.4446 & n.a. \\
%   QG & 0.5672 & 0.4527 & 5.8070 & 7.3315 & 0.3089 & 0.3036 & 0.4685 & 0.7866 \\
%   \textbf{ContrastQG} & \textbf{0.5909} & \textbf{0.4627} & \textbf{6.1282} & \textbf{7.6314} & \textbf{0.3191} & \textbf{0.3123} & \textbf{0.4769} & \textbf{0.7908} \\
%   reverse ContrastQG & 0.3185 & 0.1807 & 3.0076 & 3.3665 & 0.1610 & - & - & - \\
%   \bottomrule
%   \end{tabular}
%   }
%   \caption{\label{tab:contrastqg}The query generation performance and neural ranking performance with different weakly supervised sources (w/o MetaAdpatLTR). We only report NDCG@20 due to the space limit.}
% \end{table*}

==> Diagrams/meta_case_examples.tex <==
\begin{table*}
\centering
\small
\resizebox{\textwidth}{!}{
  \begin{tabular}{l l|l|l}
   \hline \hline
  \multicolumn{2}{l|}{\textbf{Anchor}} & \textbf{ Positive Document} & \textbf{ Negative Document} \\ 
    \hline
    1 &  \textbf{(+)} enquirer & \makecell[l]{... the national \textbf{enquirer} is the undisputed leader in the \\ \hspace{0.5em}field of celebrity journalism  in every issue of \textbf{enquirer} ...} & \makecell[l]{... login sign up search socialize and find national \textbf{enquirer} \\ \hspace{0.5em}celebrity news photos crime gossip ...} \\
    \hline
    2 & \textbf{(+)}  hilton garden inn austin  & \makecell[l]{... \textbf{hilton garden inn austin} nw hotel is in the northwest \\ \hspace{0.5em}arboretum area of austins golden triangle downtown ...} & \makecell[l]{... home about contact \textbf{austin} hotel profile search form \\ \hspace{0.5em}\textbf{austin} add your hotel area hotel rates group hotel rates ...}\\
    \hline
    3 &  \textbf{(+)} lupus nephritis & \makecell[l]{... \textbf{lupus nephritis} is an inflammation of the kidney that \\ \hspace{0.5em}is caused by systemic lupus erythematosus or sle it is...} & \makecell[l]{... what is it alternative names causes symptoms \\ \hspace{0.5em}signs treatments where to get support prognosis possible ...} \\
    \hline
    4 & \textbf{(+)} hot water dispenser  & \makecell[l]{... how to install a \textbf{hot water dispenser} an instant \textbf{hot} \\ \hspace{0.5em}\textbf{water dispenser} can be a time saver in the kitchen ...} & \makecell[l]{... pacific jumbo tissue \textbf{dispenser} medready audimated \\ \hspace{0.5em}medication \textbf{dispenser} decorative cat soap \textbf{dispenser} ...} \\
    \hline \hline
    5 & \textbf{(-)} ebv  & \makecell[l]{... homo sapiens diseases s hodgkin disease hd or \\ \hspace{0.5em}lymphoma hl malignant lymphogranuloma ...} & \makecell[l]{... most versatile fiber optics solution for the industrial \\ \hspace{0.5em}market open pdf ebrochure by \textbf{ebv} english ...} \\
    \hline
    6 & \textbf{(-)} orlando sentinel  & \makecell[l]{... \textbf{orlando sentinel} online directory links 5 bedroom \\ \hspace{0.5em}orlando rental villa 5 star hotel in \textbf{orlando} airport car ...} & \makecell[l]{... loading rss feeds allow web site content to be gathered \\ \hspace{0.5em}via feed reader software click the subscribe link to obtain ...} \\
    \hline
    7 &  \textbf{(-)} movie licensing usa & \makecell[l]{... we represent family \textbf{movie} night promotional materials \\ \hspace{0.5em}program ideas company profile frequently asked ...} & \makecell[l]{... \textbf{movie licensing usa} is a division of swank motion pictures \\ \hspace{0.5em}inc and has served as the non theatrical distributor of ...} \\
    \hline
    8 & \textbf{(-)} you tube  & \makecell[l]{... \textbf{you tube} obama speech \textbf{you tube} rick astley \textbf{you tube} \\ \hspace{0.5em}step up 2 you tube iron man \textbf{you tube} xanadu search ...} & \makecell[l]{... yuku free message boards username or e mail password \\ \hspace{0.5em}forgot password sign up search pishpishrialniz kudos ...} \\
    \hline \hline
  \end{tabular}}
  \caption{\label{tab:case}
      Examples of weak supervision data during experiments described in \ref{sec:appendix:case_study}. The directions of their meta-gradients in the last stage are marked in the parenthesis (+/-). The document snippets are manually selected.
  }
\end{table*}


==> Diagrams/meta_loop.tex <==
\begin{figure}[t]
  \centering
    \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{Figures/meta_loop1.pdf}
    \caption{Constructing the Meta Forward Loop.\label{fig:meta_forward}}
    \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{Figures/meta_loop2.pdf}
    \caption{Weighting Data with Meta-Gradient.\label{fig:meta_backward}}
    \end{subfigure}
\caption{\label{fig:meta_loop} An illustration of meta learning process for Few-shot Neu-IR, including the meta forward loop construction (a) and the data weight learning by back-propagating the meta-gradients (b).
}
\end{figure}

% \begin{figure}[t]
%   \centering
%     \begin{subfigure}[t]{\linewidth}
%     \includegraphics[width=\textwidth]{Figures/meta_loop_1.pdf}
%     \caption{Constructing the Meta Forward Loop.\label{fig:meta_forward}}
%     \end{subfigure}
%     \begin{subfigure}[t]{\linewidth}
%     \includegraphics[width=\textwidth]{Figures/meta_loop_2.pdf}
%     \caption{Weighting Data with Meta-Gradient.\label{fig:meta_backward}}
%     \end{subfigure}
% \caption{\label{fig:meta_loop} An illustration of Meta Learning to Weight (\metaweight{}) for Few-shot Neu-IR, including the meta forward loop construction (a) and the data weight learning by back-propagating the meta-gradients (b).
% }
% \end{figure}

% \includegraphics[width=0.48\textwidth]{Figures/meta_loop_1.pdf}
% \caption{Constructing the Meta Forward Loop.\label{fig:meta_forward}}
% \includegraphics[width=0.48\textwidth]{Figures/meta_loop_2.pdf}
% \centering
% \caption{Weighting Data with Meta-Gradient.\label{fig:meta_backward}}

==> Diagrams/query_num.tex <==
\begin{figure}[t]
 \centering
    \begin{subfigure}[t]{0.455\linewidth}
        \includegraphics[width=\textwidth]{Figures/query_num.pdf}
        \caption{Effectiveness.\label{fig:query_num}}
    \end{subfigure}
    \begin{subfigure}[t]{0.455\linewidth}
        \includegraphics[width=\textwidth]{Figures/run_time.pdf}
        \centering
        \caption{Efficiency.\label{fig:run_time}}
    \end{subfigure}
\caption{\label{fig:few_shot}
Effectiveness and efficiency of selective weak supervision methods. The number of available few-shot target queries with relevance labels is shown on X-Axes. 
The Y-Axes list the ranking accuracy on a ClueWeb09 testing fold in the Fine-Tune setting (a) and the logarithmic overhead in estimating data importance over vanilla All Anchor weak supervision (b).}
\end{figure}




==> Diagrams/rank_robust.tex <==
\begin{figure}[t]
    % \begin{subfigure}[t]{0.48\linewidth}
    %     \includegraphics[width=\textwidth]{Figures/cknrm_rank_robust.pdf}
    %     \caption{Conv-KNRM.\label{fig:cknrm_rb}}
    % \end{subfigure}
    \centering
        \includegraphics[width=0.25\textwidth]{Figures/bert_rank_robust.pdf}

\caption{\label{fig:bert_rb}
Ranking accuracy at different training steps.
The NDCG@20 in the Fine-Tune setting on a ClueWeb09 testing fold is plotted (Y-Axes) along with different training steps (X-Axes). Note ReInfoSelect starts higher as we warmed it up with All Anchor trained ranker weights, which is not needed in \meta{}.
}
\end{figure}

